Data-Centric Green AI: An Exploratory Empirical Study

With the growing availability of large-scale datasets, and the popularization of affordable storage and computational capabilities, the energy consumed by AI is becoming a growing concern. To address this issue, in recent years, studies have focused on demonstrating how AI energy efficiency can be improved by tuning the model training strategy. Nevertheless, how modifications applied to datasets can impact the energy consumption of AI is still an open question. To fill this gap, in this exploratory study, we evaluate if data-centric approaches can be utilized to improve AI energy efficiency. To achieve our goal, we conduct an empirical experiment, executed by considering 6 different AI algorithms, a dataset comprising 5,574 data points, and two dataset modifications (number of data points and number of features). Our results show evidence that, by exclusively conducting modifications on datasets, energy consumption can be drastically reduced (up to 92.16%), often at the cost of a negligible or even absent accuracy decline. As additional introductory results, we demonstrate how, by exclusively changing the algorithm used, energy savings up to two orders of magnitude can be achieved. In conclusion, this exploratory investigation empirically demonstrates the importance of applying data-centric techniques to improve AI energy efficiency. Our results call for a research agenda that focuses on data-centric techniques, to further enable and democratize Green AI.

==> Green AI (1)/abstract.tex <==


\begin{abstract}
With the popularization of affordable storage capabilities, computational power, and data availability, 

artificial intelligence is experiencing an unprecedented level of adoption. As datasets grow in sizes, and new complex application domains emerge, the energy consumption of artificial intelligence algorithms is becoming a growing concern. 

background
objective
method
results
conclusion

% The current trend in training AI is to use more and more data to give greater precision in elaborating prediction models. This increase of the size of the dataset translates into more and more processing which leads to an increase in the energy use that is necessary to process all the data. The energy consumption is currently not a factor considered in training AI.
% %
% %%%% Another draft %%%%%%%%
% %Context
% The size of datasets used in training AI is getting bigger and bigger as a result of the quest to achieve more and more accuracy in AI models. 
% %
% %Problem
% More data in the dataset means more processing computation. More computation generates an increase of the energy consumption needed. 
% %
% %Why is it a problem?
% The energy consumption is a key element in the transformation towards a sustainable society. The goal is to preserve the available resources and reduce the overall consumption of energy. So, the goal is to move forward technologies that consume less energy. In that way, the current state of the ever growing size of data used in AI seems to go the opposite way from a more sustainable society.
% %
% %Solution
% We propose to look at the possible impacts the dataset can have on the energy consumption made by the training process of AI models. We present the relationship between the properties of the dataset and the energy consumption of training the associated AI models.
% %
% %Why a solution?
% With insight on how the properties and the energy consumption are related, we aim to raise awareness about the choices made by AI developers regarding the properties of the datasets when training AI models. That way, the goal is to prevent a higher energy consumption for generating AI models with the same range of accuracy.
% %
% %Results
% We explore and study the aforementioned relationships between the dataset's properties and energy consumption in the case of an open source ML project. We compare the energy consumption of the training process in different cases corresponding to different formatting of the dataset (i.e., …..).
% We show that …… 



% \jsnote{ mention possible trade-off between accuracy and energy consumption? In some cases, a slight decrease of accuracy can be accepted as it can lead to a consequent decrease of energy consumption in the training process. }

%
\end{abstract}

==> Green AI (1)/introduction.tex <==
\section{Introduction}
%AI more and more used
 We live in the era of artificial intelligence (AI): new intelligent technologies are emerging every day to change people's lives. Many organizations identified the massive potential of using intelligent solutions to create business value. Hence, in the past years, the \textit{modus operandi} is collecting as much data as possible so that no opportunity is missed. Data science teams are constantly looking for problems where AI can be applied to existing data to train models that can provide more personalized and optimized solutions to their operations customers and operations~\cite{haakman2021ai}.


%Green AI
Nevertheless, the energy consumption of developing AI applications is starting to be a concern.
Previous studies observed that AI-related tasks are particularly energy-greedy~\cite{Strubell2019,Lacoste2019}.
In fact, since 2012, the amount of computing used for AI training has been doubling every 3.4 months~\cite{amodey2018ai}. Controversy has risen around particular machine learning models that have been estimated to consume the energy equivalent of a trans-American flight~\cite{Bender2021}.
Hence, a new subfield is emerging to make the development and application of AI technologies environmentally sustainable: \emph{Green AI}~\cite{Schwartz2020}.

%t the training procedure emitted 284t of cot2

%Data-centric AI
On a related note, the current research practice of collecting massive amounts of data is not necessarily yielding better results. Being able to collect high-quality data is more important than collecting big data -- a trend coined as \emph{Data-centric AI}\footnote{Understanding Data-Centric AI: \url{https://landing.ai/data-centric-ai/}. Accessed 24th January 2022.}. Instead of creating learning techniques that squeeze every bit of performance, data-centric AI focuses on leveraging systematic, reliable, and efficient practices to collect high-quality data. 

%Green data-centric AI
Therefore, in this study, we conduct an exploratory empirical study on the intersection of Green AI and Data-centric AI. We investigate the potential impact of modifying datasets to improve the energy consumption of training AI models. In particular, we focus on machine learning, the branch of AI that deals with the automatic generation of models based on sample data -- machine learning and AI are used interchangeably throughout this paper.
In addition to investigating the energy impact of dataset modifications, we also analyze the inherent trade-offs between energy consumption and performance when reducing the size of the dataset -- either in the number of data points or features. Moreover, the analysis is performed in six state-of-the-art machine learning models applied in the detection of Spam messages.

% Results
Our results show that feature selection can reduce the energy consumption of model training up to 76\% while preserving the performance of the model. The improvement in energy efficiency is more impressive when reducing the number of data points: up to 92\% in the case of Random Forest. However, in this case, it is not cost-free: the trade-off between energy and performance needs to be considered. Finally, we also show that KNN tends to be the most energy-efficient algorithm, while ensemble classifiers tend to be the most energy greedy.

% Implications

This paper provides insights to define the most relevant and energy-efficient modifications of datasets used during the development of the AI models while ensuring minimal accuracy loss. We argue that more research in Data-centric AI will help more practitioners in developing green AI models.
To the best of our knowledge, this is the first study to explore the potential of preprocessing data to reduce the energy consumption of AI. 

% rep package
The entirety of our experimental scripts and results are made available with an open-source license, to enable the independent verification and replication of the results presented in this study: \url{https://github.com/GreenAIproject/ICT4S22}.

% remainder
% Outline of the paper
The remainder of this paper is structured as follows. Section~\ref{sec:relatedWork} presents the related work on the energy consumption of Artificial Intelligence models. Section~\ref{sec:studyDesign} details the overall approach and the study design. Section~\ref{sec:results} describes the results of the experimentation according to the different dataset modifications, and Section~\ref{sec:discussion} presents the related discussion. The threats to the validity of this study are thoroughly analyzed in Section~\ref{sec:threats}. Finally, Section~\ref{sec:conclusion} documents our conclusions and future work.

%\jsnote{General question about the section/paper: We say that we are looking at the energy consumption wrt AI but not really the purpose of it. Okay, we want to know that factors impact it but not the end goal. Do we ant to say that we would like to inform the practitioners of what factors impact the energy consumption in order for them to chose what practises or what "levels" of factors to do, in order to consume minimal energy WHILE ensuring a minimal impact on the accuracy of their model? I think we need to emphasise the importance of the fact that we want to maintain the accuracy of the AI model within an acceptable range. I don't know in which section to put it though.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%template%%%%%%%%%%%%%%%

